SZ3: A Modular Framework for Composing Prediction-Based Error-Bounded Lossy Compressors

Today's scientific simulations require a significant reduction of data volume because of extremely large amounts of data they produce and the limited I/O bandwidth and storage space. Error-bounded lossy compressor has been considered one of the most effective solutions to the above problem. In practice, however, the best-fit compression method often needs to be customized/optimized in particular because of diverse characteristics in different datasets and various user requirements on the compression quality and performance. In this paper, we develop a novel modular, composable compression framework (namely SZ3), which involves three significant contributions. (1) SZ3 features a modular abstraction for the prediction-based compression framework such that the new compression modules can be plugged in easily. (2) SZ3 supports multialgorithm predictors and can automatically select the best-fit predictor for each data block based on the designed error estimation criterion. (3) SZ3 allows users to easily compose different compression pipelines on demand, such that both compression quality and performance can be significantly improved for their specific datasets and requirements. (4) In addition, we evaluate several lossy compressors composed from SZ3 using the real-world datasets. Specifically, we leverage SZ3 to improve the compression quality and performance for different use-cases, including GAMESS quantum chemistry dataset and Advanced Photon Source (APS) instrument dataset. Experiments show that our customized compression pipelines lead to up to 20% improvement in compression ratios under the same data distortion compared with the state-of-the-art approaches.

==> tex/predictors.tex <==
\section{Predictors}
\label{sec:predictors}
{\color{red} I would like to introduce the pre-mentioned 4 default predictors}

We introduce the 4 pre-mentioned predictors and their corresponding error estimation mechanisms in this section.

\subsection{Lorenzo Predictor}

\subsection{Regression-based Predictor}

\subsubsection{}
\subsubsection{Prediction Workflow}
The prediction workflow of a linear-regression-based predictor is displayed in Fig.~\ref{}.

\textbf{Derivation of Regression Coefficients:}~In what follows, we derive the regression coefficients for a dataset with $m$ dimensions ($n_1$$\times$$n_2$$\times$$\cdots$$\times$$n_m$) from a generic perspective, which can be easily extended to block-wise situations. The value at position $\boldsymbol{x} = (i_1, \dots, i_m)$ is denoted as $f(\boldsymbol{x}) = f_{i_1\dots i_m}$, where $i_j$ is its index along each dimension. We also denote $f^{(r)}$ as the linear regression prediction. Then the linear regression model can be built as:
\vspace{-1.5mm}
$$
\vspace{-1.5mm}
	f^{(r)}(\boldsymbol{x} ) = \boldsymbol{x}^T\boldsymbol{\beta} + \alpha
$$
where $\boldsymbol{\beta}$ = ($\beta_1$,$\dots$,$\beta_m$) denotes the slope coefficient vector and the constant $\alpha$ is the intercept coefficient. 
By redefining $\boldsymbol{x'} = (1, i_1, \dots, i_m)$ and $\boldsymbol{\beta'}$ = $($$\beta_0$=$\alpha$,$\beta_1$,$\dots$,$\beta_m$$)$, the formula above can be rewritten as:
\vspace{-1.5mm}
$$
\vspace{-1.5mm}
	f^{(r)}(\boldsymbol{x'} ) = \boldsymbol{x'}^T\boldsymbol{\beta'} 
$$
Since each data point corresponds to a position $\boldsymbol{x}$ and its value $f(\boldsymbol{x})$, the objective of the regression model is to minimize the squared error (SE) between predicated and original values:
\vspace{-1.5mm}
$$
\vspace{-1.5mm}
	SE = \sum_{\boldsymbol{x'} \in \{(1, i_1, \dots, i_m) | 0 \leq i_j < n_j\}} (\boldsymbol{x'}^T\boldsymbol{\beta'}  - f_{i_1\dots i_m})^2
$$
This is a convex function, and its optimal can be obtained by derivation. The derivation over each element in $\boldsymbol{\beta'}$ will result in a linear system of $m$ unknowns. By solving the linear system, the optimal solution can be achieved as:
\vspace{-1.5mm}
\begin{equation}
\label{eq:betasol}
\vspace{-1.5mm}
	\boldsymbol{\beta'} = (X^TX)^{-1}X^Ty 
\end{equation}
$X$ is the full permutation of \{$i_1$,$i_2$,$\cdots$,$i_m$\}, where $i_j$$\in$\{0,1,$\cdots$,$n_j$$-$1\}, and $y$ is the sequence of the corresponding data values ($f_{00\dots0}$,$f_{00\dots1}$,$\cdots$,$f_{(n_1-1)(n_2-1)\dots (n_m-1)}$). 

Since $X$ is a \{$\prod_{1 \leq i \leq m}{n_i}$\}$\times$$(m+1)$ matrix, 
computing the closed-form solution (\ref{eq:betasol}) is very expensive. However, we can derive the solution to a simple form, significantly reducing the computation cost. Let us take a 3D dataset as an example to describe our method, which can be extended to datasets with higher dimensions easily without loss of generality. 

\begin{lemma}
The regression coefficients of a 3D dataset with dimensions $n_1$, $n_2$, $n_3$  can be calculated as:
\vspace{-1.5mm}
\begin{equation}
\label{eq:thm1sol}
\vspace{-1.5mm}
\left\{ \begin{array}{l}
 \beta_1 = \frac{6}{n_1n_2n_3(n_1 + 1)}(\frac{2V_x}{n_1 - 1} - V_0) \\ 
 \beta_2 = \frac{6}{n_1n_2n_3(n_2 + 1)}(\frac{2V_y}{n_2 - 1} - V_0) \\ 
 \beta_3 = \frac{6}{n_1n_2n_3(n_3 + 1)}(\frac{2V_z}{n_3 - 1} - V_0) \\ 
 \beta_0 = \frac{V_0}{n_1n_2n_3} - (\frac{n_1 - 1}{2}\beta_1 + \frac{n_2 - 1}{2}\beta_2 + \frac{n_3 - 1}{2}\beta_3) \\ 
 \end{array} \right.
\end{equation}
{
\small
\begin{align*}
\text{where } V_{0} = \sum_{i=0}^{n_1 - 1} \sum_{j=0}^{n_2 - 1} \sum_{k=0}^{n_3 - 1}f_{ijk}, \quad  V_{x} = \sum_{i=0}^{n_1 - 1} \sum_{j=0}^{n_2 - 1} \sum_{k=0}^{n_3 - 1}i*f_{ijk}, \\
V_{y} = \sum_{i=0}^{n_1 - 1} \sum_{j=0}^{n_2 - 1} \sum_{k=0}^{n_3 - 1}j*f_{ijk}, \quad 
V_{z} = \sum_{i=0}^{n_1 - 1} \sum_{j=0}^{n_2 - 1} \sum_{k=0}^{n_3 - 1}k*f_{ijk}.
\end{align*}
}
\end{lemma}
\begin{IEEEproof}
By substituting the index with the coordinate values, the SE expression can be formulated as:
\begin{equation*}
SE=\sum_{i=0}^{n_1 - 1} \sum_{j=0}^{n_2 - 1} \sum_{k=0}^{n_3 - 1} {(\beta_0 + \beta_1 i + \beta_2 j + \beta_3 k - f_{ijk})^2}
\end{equation*}
Deriving the coefficients then turns out to be a least-square problem aiming at minimizing the SE. This problem is equivalent to solving the following linear system, which is derived by setting all the partial derivatives of SE over the coefficients to $0$:
{
\small
$$
	\sum_{i=0}^{n_1 - 1} \sum_{j=0}^{n_2 - 1} \sum_{k=0}^{n_3 - 1}
	\begin{bmatrix}
	{1} & i & j & k\\
	{i} & i^2 & ij & ik \\
	{j} & ij & j^2 & jk \\
	{k} & ik & jk & k^2 
	\end{bmatrix}
	\begin{bmatrix}
	\beta_0\\
	\beta_1\\
	\beta_2\\
	\beta_3
	\end{bmatrix}		
	=
	\begin{bmatrix}
	V_0 \\
	V_x \\
	V_y \\
	V_z 
	\end{bmatrix}
$$
}
Since $\sum_{i=0}^{n - 1}{i} = \frac{n(n - 1)}{2}$ and $\sum_{i=0}^{n - 1}{i^2} = \frac{(2n - 1)n(n - 1)}{6}$, the above linear system can be simplified to:
{
\small
$$
	\begin{bmatrix}
	1 & \frac{(n_1 - 1)}{2} & \frac{(n_2 - 1)}{2} & \frac{(n_3 - 1)}{2}\\
	1 & \frac{(2n_1 - 1)}{3} & \frac{(n_2 - 1)}{2} & \frac{(n_3 - 1)}{2}\\
	1 & \frac{(n_1 - 1)}{2} & \frac{(2n_2 - 1)}{3} & \frac{(n_3 - 1)}{2}\\
	1 & \frac{(n_1 - 1)}{2} & \frac{(n_2 - 1)}{2} & \frac{(2n_3 - 1)}{3}\\
	\end{bmatrix}
    \hspace{-2mm}
	\begin{bmatrix}
	\beta_0\\
	\beta_1\\
	\beta_2\\
	\beta_3
	\end{bmatrix}		
	=
	\begin{bmatrix}
	\frac{V_0}{n_1n_2n_3} \\
	\frac{2V_x}{n_1n_2n_3(n_1 - 1)} \\
	\frac{2V_y}{{n_1n_2n_3(n_2 - 1)}} \\
	\frac{2V_z}{{n_1n_2n_3(n_3 - 1)}} 
	\end{bmatrix}
$$
}
After that, Gaussian elimination can be leveraged to transfer the linear system as follows:
{
\small
$$
	\begin{bmatrix}
	1 &\hspace{-2mm} \frac{(n_1 - 1)}{2} &\hspace{-2mm} \frac{(n_2 - 1)}{2} &\hspace{-2mm} \frac{(n_3 - 1)}{2}\\
	0 &\hspace{-2mm} 1 &\hspace{-2mm} 0 &\hspace{-2mm} 0\\
	0 &\hspace{-2mm} 0 &\hspace{-2mm} 1 &\hspace{-2mm} 0\\
	0 &\hspace{-2mm} 0 &\hspace{-2mm} 0 &\hspace{-2mm} 1\\
	\end{bmatrix}
    \hspace{-2mm}
	\begin{bmatrix}
	\beta_0\\
	\beta_1\\
	\beta_2\\
	\beta_3
	\end{bmatrix}		
	=
	\begin{bmatrix}
	\frac{V_0}{n_1n_2n_3} \\
	\frac{6}{n_1n_2n_3(n_1 + 1)}(\frac{2V_x}{n_1 - 1} - V_0) \\
	\frac{6}{n_1n_2n_3(n_2 + 1)}(\frac{2V_y}{n_2 - 1} - V_0) \\
	\frac{6}{n_1n_2n_3(n_3 + 1)}(\frac{2V_z}{n_3 - 1} - V_0)  
	\end{bmatrix}
$$
}
Then Equation (\ref{eq:thm1sol}) can be derived accordingly.
\end{IEEEproof}

\textbf{Coefficient Compression:}~

\textbf{Prediction: }~These coefficients will be used in the regression model for predicting the data accurately. Each data point with index $(i, j, k)$ will be predicted as $f^{(r)}_{ijk} = \beta_0 + i\beta_1 + j\beta_2 + k \beta_3$. Then, we will compute the difference between each predicted value $f^{(r)}_{ijk}$ and its original value $f_{ijk}$, and perform the linear-scaling quantization \cite{sz17} to convert the floating-point values to integer codes. The data size will be significantly reduced after conducting Huffman encoding on the quantization codes. 

\subsection{Composed Predictor}
\subsection{Pattern-based Predictor}

% \subsection{Transform-based Predictor}




==> tex/problem.tex <==
\section{Design overview}
\label{sec:design}

